Spectral Fusion for Identifying Early State Exclusion in Symmetric Quantum Spin Chains

Perfect state transfer (PST) in one-dimensional quantum spin chains provides a natural setting in which quantum information transport can be analyzed using spectral methods. In the single-excitation subspace, the dynamics of a chain with nearest-neighbor interactions are governed by a Jacobi matrix, allowing questions of state transfer to be formulated in terms of eigenvalue distributions and symmetry properties of eigenvectors. In this work, we investigate the phenomenon of \emph{early state exclusion} (ESE), whereby the overlap of the time-evolved state with the initial state vanishes at a time strictly earlier than the first occurrence of perfect state transfer. Building on earlier constructions of Hamiltonians exhibiting PST with and without ESE, we provide explicit Jacobi matrix realizations for arbitrary odd-length chains and establish general conditions under which ESE occurs or does not occur. We propose the process of \emph{spectral fusion} (SF) to build infinite families of such Hamiltonians. These results broaden the known class of spin chains displaying early state exclusion and further clarify the role of spectral structure of the Hamiltonians.

==> info.tex <==
% Edit the following

% Personal information
\newcommand{\myname}{Valentin Garcia} % Your name (e.g. "John Smith")
\newcommand{\mytitle}{Undergraduate Student\\Corresponding Author} % Your title (e.g. "Applicant")
\newcommand{\myemail}{valentin{\textunderscore}garcia@brown.edu} % Your email (e.g. "me@mydomain.com")
\newcommand{\mylinkedin}{johndoe} % Your LinkedIn profile name (e.g. "myname")
\newcommand{\myphone}{123.456.7890} % Your phone number (e.g. "123.456.7890")
\newcommand{\mylocation}{Brown University, Providence, RI} % Your general location (e.g. "PNW, USA")
\newcommand{\recipient}{Editorial Board} % The recipient (e.g. "Hiring Manager")
\newcommand{\greeting}{Dear} % The greeting to use (e.g. "Dear")
\newcommand{\closer}{Kind Regards} % The closer to use (e.g. "Kind Regards")

% Company information
\newcommand{\company}{SIAM Undergraduate Research Online (SIURO) } % The company (e.g. "Microsoft Corporation")
\newcommand{\street}{3600 Market Street \\ 6th Floor} % The company's street address (e.g. "1 Microsoft Way")
\newcommand{\city}{Philadelphia} % The company's city (e.g. "Redmond")
\newcommand{\state}{PA} % The company's state prefix (e.g. "WA")
\newcommand{\zip}{19104} % The company's zip code (e.g. "98052")
